On Linear Time Decidability of Differential Privacy for Programs with Unbounded Inputs

We introduce an automata model for describing interesting classes of differential privacy mechanisms/algorithms that include known mechanisms from the literature. These automata can model algorithms whose inputs can be an unbounded sequence of real-valued query answers. We consider the problem of checking whether there exists a constant $d$ such that the algorithm described by these automata are $d\epsilon$-differentially private for all positive values of the privacy budget parameter $\epsilon$. We show that this problem can be decided in time linear in the automaton's size by identifying a necessary and sufficient condition on the underlying graph of the automaton. This paper's results are the first decidability results known for algorithms with an unbounded number of query answers taking values from the set of reals.

==> Section4_decidability.tex <==

% !TEX root =  main.tex
\section{Decidability of Differential Privacy for {\dipautos}}
\label{sec:decidability}

%Our proof of decidability of checking differential privacy of an automata is based on showing 
We shall now establish necessary and sufficient conditions for a {\dipa} $\cA$ to be 
differentially private.  These conditions will turn out to be simple graph-theoretic conditions
on the ``underlying graph" of the   {\dipa} $\cA$, and shall be used to establish the  decidability of the differential privacy problem.
We start by formalizing these graph-theoretic properties.

\red{0th and first}


\begin{definition}
Let  $\cA$
be a {\dipautos}. 
A path $\rho$ of length $n>0$
%$\rho=\defexec$, where $n>0$,
%A path $(q_i,a_{i},o_{i},f(a_{i},\epsilon),c_i,A_i,q_{i+1})$, for
%$i=0,...,n-1$
is called a {\em {\criticalpath}} if there exist
values $i,j$ such that $0\leq i<j<n$ such that the $i$-th transition of $\rho$
is an assignment
transition and the Boolean condition of $j$-th transition is  $\lttest$ or $\getest.$ 
If  the {\criticalpath} $\rho$ is a cycle then we call $\rho$ a {\em {\criticalcycle}}.  
\end{definition}

Intuitively, in a {\criticalpath}, the
variable $\rvar$ is assigned a value in some transition which  is used in the
condition of a later transition. 
Observe that if a path is \critical,
then all paths equivalent to it are also {\critical}. As we shall see later, the presence of a {\criticalcycle} rules out the possibility of a {\dipa} being differentially private.  
\begin{example}
\label{ex:leakcycle}
Consider the {\dipa} $\sortauto$ from Example~\ref{ex:autos} on Page~\pageref{ex:autos}. The cycle 
$q_1\trns{a_1,\bot}q_1\trns{a_2,\bot}q_1$ is a {\criticalcycle} for any $a_1,a_2$ as the 0th transition is an assignment transition  and the first transition has Boolean condition $\lttest.$
\end{example}
\begin{definition}
A cycle of a {\dipa} $\cA$ is called an
{\lcycle} (respectively,  {\gcycle}) if it has a transition  whose Boolean condition  is  $\lttest$ (respectively, $\getest$).

We say that a path  of a {\dipa} $\cA$
 is an {\alpath} (respectively, {\agpath}) if all the assignment
transitions on it have the condition $ \lttest$ (respectively,
$\getest$).

\end{definition}

Observe that a cycle can be both an {\lcycle} as well as a {\gcycle}. Further, a path with no assignment transitions (including the empty path) is simultaneously 
both an {\alpath} and an {\agpath}.

%\begin{definition}
%We say that a path  of a {\dipa} $\cA$
% is an {\alpath} (respectively, {\agpath}) if all the assignment
%transitions on it have the condition $ \lttest$ (respectively,
%$\getest$).
%\end{definition}


\begin{definition}
Consider a pair of cycles $(C,C')$ in a {\dipa} $\cA.$ We call the pair $(C,C')$ a {\em
  {\criticalpair}} if one of the following two conditions is satisfied.
\begin{enumerate}
\item  $C$ is an {\lcycle}, $C'$ is a {\gcycle} and there is an
  {\agpath} 
  from a state in $C$ to a state in $C'.$ 

\item  $C$ is a {\gcycle}, $C'$ is an {\lcycle} and there is an
  {\alpath} from a state in $C$ to a state in $C'.$ 
\end{enumerate}
\end{definition}


Observe that if $C$ is an {\lcycle} as well as a {\gcycle}, then the
pair $(C,C)$ is a {\criticalpair} with the empty path connecting 
$C$ to itself. Also, if $(C,C')$ is a {\criticalpair}, then for any
$C_1,C_2$ that are equivalent to $C,C'$ respectively, the pair
$(C_1,C_2)$ is also a {\criticalpair}. The presence of a {\criticalcycle} rules out the possibility of a {\dipa} being differentially private. 

\begin{example}
\label{ex:leakingpair}
Consider the {\dipa} $\svtpauto$ from Example~\ref{ex:autos} on Page~\pageref{ex:autos}. The cycle $C=q_1\trns{a_1,\bot}q_1$ is an {\lcycle} for any $a_1$ and the cycle $C'=q_2\trns{a_2,\top}q_2$ is a {\gcycle} for any $a_2.$ The path $q_1\trns{a_3,\top}q_2$ is an {\agpath} from $C$ to $C'.$ Hence $(C,C')$ is a {\criticalpair}.
\end{example}

\red{Need to define reachability}

If $\cA$ does not have any {\criticalcycle}s and {\criticalpair}s then $\cA$ will be differentially private. We shall call such {\dipautop} well-formed:
\begin{definition}
A {\dipa} $\cA$ is said to be {\em well-formed} iff it has no
{\criticalcycle} that is reachable from the initial state and it has no
{\criticalpair} of cycles $(C,C')$ where $C$ is reachable from the
initial state of $\cA$.
\end{definition}

We have the following theorem which we shall establish shortly. 
\begin{theorem}
\label{thm:main}
A {\dipa} $\cA$ is 
 differentially private iff it is well-formed.  
\end{theorem}

We get as a corollary of Theorem~\ref{thm:main} that the problem of checking whether a {\dipa} $\cA$ is differentially private can be checked using graph-theoretic algorithms. 
\begin{corollary}
The problem of checking whether a {\dipa} $\cA$ is differentially private is decidable in time linear in the number of states of $\cA$. 
\end{corollary}
\begin{proof}
We describe a linear time algorithm that checks whether a {\dipa} $\cA$ is well-formed. The statement of Corollary then follows from Theorem~\ref{thm:main}.  
The algorithm proceeds as follows. Given the {\dipa} $\cA=\defaut$, it constructs an edge-labeled directed graph $\cG$ as follows. The vertices of $\cG$ is $Q$, the set of states of $\cA.$ There is an edge from vertex $p$ to vertex $q$ labeled $(c,b)$ iff there is an output $o$ such that $\delta(p,c)=(q,o,b).$  Without loss of generality, we assume that all states of $\cG$ are reachable from $\qinit.$ The graph $\cG$ can be constructed in linear time. 

Using Depth-First-Search on the graph $\cG$ the algorithm constructs the  the strongly connected components of $\cG$ and constructs the component graph $\cG_{\mathsf{com}}.$  It is easy to see that $\cA$ has a {\criticalcycle} if and only if $\cG$ has a strongly connected component that has an edge labeled $(c,\true)$ and an edge labeled $(c',b')$ for some $c,b'$ and $c'\ne \true.$ The algorithm checks for the latter condition and outputs NO if it finds that $\cA$ has a {\criticalcycle}.

If $\cA$ does not have a critical cycle then the algorithm proceeds to check whether $\cA$ has a {\criticalpair} as follows. 


\red{Complete the proof}

 \end{proof}

\red{Need to make the statement about parameter function}


\subsection{Necessary Condition for Differential Privacy}

We shall now show that if a {\dipa} $\cA$ is not well-formed then it is not $d\epsilon$-differentially private for any $d>0$. 
We start by considering the case when $\cA$ has a {\criticalcycle.} The intuition behind this result is that
each time a {\criticalcycle} $C$ is executed, it incurs a cost that is asymptotically linear in the parameter $\epsilon$. 
Thus, given  $d,$ we can always find an  $\ell$ and an $\epsilon$ such that executing the cycle $\ell$ times 
exhausts the privacy budget $d\epsilon.$ This intuition requires careful analysis and is captured in the following Lemma, whose non-trivial proof is given in
Appendix~\ref{app:if1main}.
%Lemmas \ref{lem:if1main} and \ref{lem:if2main} together prove that if
%$\cA$ is not well-formed then it is not differentially private.

%Lemma \ref{lem:onlyifmain} shows that if $\cA$ is well-formed then it
%is differentially private.


\begin{lemma}
\label{lem:if1main}
A  {\dipa} $\cA $ is 
not differentially private if  it has a {\criticalcycle}  reachable from its initial state.
\end{lemma}
\red{Do we need a proof sketch}

We now discuss the intuition behind the case when $\cA$ has no {\criticalcycle}s, but has a {\criticalpair} of cycles $(C,C')$ such that $C$ is reachable from initial state. Assume that $C'$ 
 is a {\gcycle}. The case when $C'$ is a {\lcycle} is symmetric. Let $y$ be the stored value of  $\rvar$ when $C'$ starts executing (which does not change during the execution of $C'$ as $C'$ is not a {\criticalcycle}). If $y>0,$ 
then executing $C'$ incurs a privacy cost linear in the parameter $\epsilon.$ Executing $C'$ $\ell$ times would thus exhaust the privacy budget $d\epsilon$ for large $\ell$ if $y>0.$
Similarly, executing  the {\lcycle} $C$ $\ell$ times also exhausts the privacy budget $d\epsilon$ for large $\ell$ if the stored value of $\rvar \leq 0$ during the execution of $C.$ 
Consider the path in which $C$ is repeated $\ell$ times and upon exiting follows the 
{\agpath} to $C'$ which is executed $\ell$ times. The {\agpath} condition now ensures that privacy budget $d\epsilon$ gets exhausted for every possible initial stored value of $\rvar$ for large $\ell$. This intuition is is captured in the following Lemma, whose non-trivial proof is given in
Appendix~\ref{app:if2main}.

\begin{lemma}
\label{lem:if2main}
A  {\dipa} $\cA$ is 
not differentially private if  it has a {\criticalpair} of cycles $(C,C')$ such that $C$ is reachable from the initial state of $\cA.$   

\end{lemma}


%\begin{proof}
%
%Let $\cA= \defaut.$ Assume that $\cA$ has a {\criticalcycle} reachable from the state $\qinit.$
%We give the proof first assuming that all states of $\cA$ are input states. Later we will show how we can modify the 
%construction for automata that have both input and non-input states.
%
%Let $\absexec=\absexecl{m+n}$  for $k=0,\ldots,m+n-1$ be an \red{abstract path} such that $q_0=\qinit$, $q_m=q_{m+n}$, and the  final $n$ transitions of $\rho$, i.e., the abstract path 
% $C=\absexecsf{m}{m+n}$ is a
%{\criticalcycle}. 
%
% Let $t_k$ be the \red{$k$-th transition} of $\absexec$ and $c_k$ be the \red{Boolean condition} of the $k$-th transition. 
%  Further, let $d_k$ and $\mu_k$ be such that $\parf(q_k) = (d_k,\mu_k)$ for each $k.$
% \red{Without loss of generality}, we assume that
%$c_0\:=\true$ and  $t_0$ is an
%assignment transition.
%Let $i,j$ be the smallest integers such that $m\leq
%i<j<m+n$ and the following properties are satisfied: (a)   
%$t_i$ is an assignment transition, (b) $c_j\neq \true$ and (c) for every
%$k_1$ such that $i<k_1<j$, $t_{k_{1}}$ is a non-assignment transition and
%$c_{k_{1}}=\true.$ We fix $i,j$ as above.
%Consider any integer $\ell>0$. We defined an abstract path $\absexec_\ell$ starting
%from $\qinit$ by repeating the cycle $t_m,...,t_{m+n-1}$, $\ell$
%times. Formally, $\absexec_\ell=\absexecl{m+\ell n}$ such that 
%$q_k=q_{k-n}$ and $o_k=q_{k-n}$ for $m+n\leq
%k\leq m+\ell n.$
%
%
%%Formally, $\absexec_{\ell}\:=(t_0,...,t_k...,t_{m+\ell n-1})$ 
%%, where $t_k\:=t_{k-n}$ for $m+n\leq
%%k<m+\ell n.$
%
%
%
%%Let $\rho=\execl{m+n}$ for $k=0,\ldots,m+n-1$ be a path such that $q_0=\qinit$, $q_m=q_{m+n}$ such that the 
%%final $n$ transitions of $\rho$, i.e., the execution $C=\execsf{m}{m+n}$ is a
%%{\criticalcycle}. 
%
%
%%Let $t_k\:=(q_k,a_k,o_k,f(a_k,\epsilon),c_k,A_k,q_{k+1})$, for
%%$k=0,...m+n-1$, be a path such that $q_0=\qinit$, $q_m=q_{m+n}$  and
%%the sequence of transitions
%%$t_m,...,t_{m+n-1}$, is a
%%{\criticalcycle}. Without loss of generality we assume that
%%$c_0\:=\true$ and  $t_0$ is an
%%assignment transition.
%%Let $i,j$ be the smallest integers such that $m\leq
%%i<j<m+n$ and the following properties are satisfied: (a)   
%%$t_i$ is an assignment transition, (b) $c_j\neq \true$ and (c) for every
%%$k_1$ such that $i<k_1<j$, $t_{k_{1}}$ is a non-assignment transition and
%%$c_{k_{1}}=\true.$ We fix $i,j$ as above.
%%Consider any integer $\ell>0$. We defined a path $\absexec_{\ell}$ starting
%%from $\qinit$ by repeating the cycle $t_m,...,t_{m+n-1}$, $\ell$
%%times. Formally, $\absexec_{\ell}\:=(t_0,...,t_k...,t_{m+\ell n-1})$ 
%%, where $t_k\:=t_{k-n}$ for $m+n\leq
%%k<m+\ell n.$
%
%Now, given $\ell>0$, we define two neighboring input sequences
%$\inalphaseq(\ell)=\inalpha_0\cdots \inalpha_{m+\ell n-1}$ and $\inbetaseq(\ell)=\inbeta_0\cdots \inbeta_{m+\ell n-1}$ each of length $m+\ell n.$  
%%Both $\inalphaseq(\ell),\inbetaseq(\ell)$ are
%%given by the sequences $\inalpha_k$ and $\inbeta_k$,$k=0,...,m+\ell n-1.$
%
%The sequence $\inalphaseq(\ell)$ is chosen so that all the conditions in
%the transitions of $\absexec_{\ell}$ are satisfied with joint probability $>\frac{1}{2}$ 
%\red{for large $\epsilon$}.
%The input $\inalpha_0=0$ and for $0<k<m+\ell n$, $\inalpha_k$ is defined
%inductively as given below: let $k'<k$ be the largest
%integer such that $t_{k'}$ is an assignment transition, then $\inalpha_k$ is
%given as follows: if  $c_k$ is the condition ${\getest}$ then
%$\inalpha_k\:=\mu_{k'}-\mu_{k}+\inalpha_{k'}+1$, otherwise $\inalpha_k\:=\mu_{k'}-\mu_{k}+\inalpha_{k'}-1.$ Let
%$\outgammaseq(\ell)$ be the sequence of outputs given by $o_k$, for $0\leq
%k<m+\ell n.$  
%
%Now, consider any $k$, $0\leq k<m+\ell n$, such that
%$c_k\neq \true$ and fix it. Let $k'<k$ be the largest integer such that $t_{k'}$ is
%an assignment transition. Let $X_{k'},X_{k}$ be the two random
%variables with distributions given by
%$\Lap{d_{k'}\epsilon,\inalpha_{k'}}$ and
%  $\Lap{d_{k}\epsilon,\inalpha_{k}}.$  Let
%    $Y_k$ denote the random variable denoting the $k^{th}$ output of $\absexec$ on
%    the input sequence $\inalphaseq(\ell).$ 
% Now
%    consider the case when $c_k$ is ${\getest}.$ From the way, we
%    defined $\inalphaseq(\ell)$ it is the case that $\mu_k+a_k\:=\mu_{k'}+a_{k'}+1.$ Now
%    $\prbfn{Y_k\neq o_k}
%\:= \prbfn{X_k < X_{k'}}\:=\prbfn{X_k\leq X_{k'}}.$ Let $d_{\mathsf{mx}}=\max(d_k,d_{k'})$ and $d_{\mathsf{mn}} = \min (d_k,d_{k'}).$
%From Lemma \ref{lem:problessequal}, we see that 
%if $d_k\neq d_{k'}$ then 
%%$$\prbfn\{X_k \leq X_{k'}\}<
%%\frac{(\max(d_{k'},d_{k}))^2}{2((\max(d_{k'},d_{k}))^2-(\min(d_{k'},d_{k}))^2)}\eulerv{-\min(d_{k'},d_{k})\epsilon}$$
%$$\prbfn{X_k \leq X_{k'}}<
%\frac{{d_{\mathsf{mx}}}^2}{2({d_{\mathsf{mx}}}^2-{d_{\mathsf{mn}}}^2)}\eulerv{-d_{\mathsf{mn}}\epsilon}.$$
%If $k=k'$ then 
%$$\prbfn{X_k \leq
%X_{k'}}<\frac{1}{2}\eulerv{-d_{k}\epsilon}(1+\frac{d_{k}\epsilon}{2}).$$
%From the above, we see that 
%$$\prbfn{Y_k\neq o_k}\leq r
%\eulerv{-d_{\mathsf{mn}}\epsilon}(1+\frac{d_{\mathsf{mx}}\epsilon}{2})$$
%where $r$ is a constant that depends only on $\cA$ (and not on $k$).
%Now consider the case when $c_k$ is $\lttest.$ In this case,
%$\mu_k+\inalpha_k\:=\mu_k+\inalpha_{k'}-1$ and
%    $\prbfn{Y_k\neq o_k}
%\:= \prbfn{X_{k'}< X_{k}}.$ 
%By a similar analysis, in this case also,
%$$\prbfn{Y_k\neq o_k}\leq r
%\eulerv{-d_{\mathsf{mn}}\epsilon}(1+\frac{d_{\mathsf{mx}}\epsilon}{2}).$$
%
%%$$\prbfn\{Y_k\neq o_k\}\leq c
%%\eulerv{-\min(d_{k'},d_{k})\epsilon}(1+\frac{\max(d_{k},d_{k'})\epsilon}{2})$$
%%where $c$ is a constant. 
%
%Let $d_{\max}\:=\max\set{\pi_1(\parf(q))\st q\in Q}$
%and $d_{\min}\:=\min\set{\pi_1(\parf(q))\st q\in Q}.$ Then, for every $k,0\leq
%k<m+\ell n$, 
%$$\prbfn{Y_k\neq o_k}\leq r
%\eulerv{-d_{\min}\epsilon}(1+\frac{d_{\max}\epsilon}{2})$$
%%where $c$ is a constant.
%Using the union rule of probabilities, we see that,
% $$\prbfn{\exists k<m+\ell n,\: Y_k\neq o_k}\:\leq r(m+\ell n)
%\eulerv{-d_{\min}\epsilon}(1+\frac{d_{\max}\epsilon}{2}).$$ 
%Given $\ell>0$, let $\epsilon_\ell\in\Reals$, be the smallest value such that
%$$\forall \epsilon\geq \epsilon_\ell,\:  r(m+\ell n)
%\eulerv{-d_{\min}\epsilon}(1+\frac{d_{\max}\epsilon}{2}) \leq \frac{1}{2}.$$ 
%
%
%Now,  $$\red{Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)}\:=1-\prbfn{\exists k<m+\ell n,\: Y_k\neq o_k}.
%%\geq  1-  c(m+\ell n)
%%\eulerv{-d_{\min}\epsilon}(1+\frac{d_{max}\epsilon}{2}).
%$$ 
%From the construction of $\epsilon_\ell$ and above observations, we see that $\forall \epsilon\geq
%\epsilon_\ell,\:\red{Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)}\:\geq \frac{1}{2}.$
%
%Now, recall the integers $i,j$ fixed earlier. Intuitively, we define $\inbetaseq(\ell)$
%so that each of the conditions in the transitions $t_{j+\ell' n}, 0\leq
%\ell'<\ell$ are satisfied with probability $<\frac{1}{2}$.
%For each $\ell',\:0\leq \ell'<\ell$,  we let $\inbeta_{i+\ell'
%  n}\:=\inalpha_{j+\ell' n}+\mu_j -\mu_i$ and $\inbeta_{j+\ell' n}\:=\inalpha_{i+\ell' n}+\mu_i-\mu_j.$
%We observe the following. Now, for each $\ell',\:0\leq \ell'<\ell$,
%the following hold. $c_{j+\ell' n}\:=c_j\neq \true.$ If $c_{j+\ell' n}$ is the
%condition ${\getest}$ then $\inbeta_{i+\ell' n}+\mu_i\:=\inbeta_{j+\ell' n}+\mu_j+1$ since 
%$\inalpha_{j+\ell' n}+\mu_j\:=\inalpha_{i+\ell' n}+\mu_i+1.$  If $c_{j+\ell' n}$ is the
%condition $\lttest$ then $\inbeta_{j+\ell' n}+\mu_j\:=\inbeta_{i+\ell' n}+
%\mu_i+1$ since
%$\inalpha_{i+\ell' n}+\mu_i\:=\inalpha_{j+\ell' n}+\mu_j+1.$  We define $\inbeta_{i'}$, for all values of $i'<m+\ell
%n$ and $i'\notin \set{ i+\ell' n, j+\ell' n \st 0\leq \ell'<\ell}$, so
%that $\inbetaseq(\ell)$ is a neighbour of $\inalphaseq(\ell).$ It is not difficult to see
%that such a sequence $\inbetaseq(\ell)$ can be defined. For each $k, 0\leq
%k<m+\ell n$, let $U_k$ be the random variable with 
%distribution given by $\Lap{d_{q_{k}}\epsilon,\inbeta_k}$ and $Z_k$ be 
%denoting the $k^{th}$ output of $\absexec$ on
%    the input sequence $\inbetaseq(\ell).$ 
%%the random variable denoting the output value of $\cA$ on input $\inbeta_k.$  
%Let $d'\:=\min(d_{i},d_{j})$ and
%$d''\:=\max(d_{i},d_{j}).$ Now, $\prbfn{Z_j=o_j}$ is given by
%$\prbfn{U_j\geq U_i}$ if $c_j$ is the condition ${\getest}$,
%otherwise it is given by $\prbfn{U_j\leq U_i}.$ Using Lemma
%\ref{lem:problessequal} and similar reasoning as given earlier, we see that 
%$$\prbfn{Z_j=o_j}\leq
%r'\eulerv{-d'\epsilon}(1+\frac{d''\epsilon}{2})$$
%for some constant $r'.$
% For each
%$\ell',\:0<\ell'<\ell$, using the same reasoning as above with the random variables $U_{i+\ell' n},U_{j+\ell'n}$, we see that 
%$$\prbfn{Z_{j+\ell' n}=o_{j+\ell' n}}\leq
%r'\eulerv{-d'\epsilon}(1+\frac{d''\epsilon}{2}).$$
% Since for any
%$\ell_1,\ell_2$ such that $0\leq\ell_1< \ell_2<\ell$, the random
%variables $U_{i+\ell_1 n},U_{j+\ell_1 n}$ are independent of
%$U_{i+\ell_2 n},U_{j+\ell_2 n}$,
%we see that 
%$$\prbfn{\forall \ell',0\leq \ell'<\ell,\:Z_{j+\ell'
%  n}=o_{j+\ell' n}}\leq {r'}^\ell \eulerv{-d'\ell
%  \epsilon}(1+\frac{d''\epsilon}{2})^\ell.$$
%Thus,
%$$\prbfn{\forall k, 0\leq k<m+\ell n,
%Z_k=o_k}\leq  {r'}^\ell \eulerv{-d'\ell
%  \epsilon}(1+\frac{d''\epsilon}{2})^\ell.$$
%The LHS of the above equation is exactly
%\red{$Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)$.}
%
%Thus,  for any $\ell>0$, 
%$$\forall \epsilon\geq \epsilon_\ell,\:
%\frac{\red{Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)}}{\red{Pr(\inbetaseq(\ell),\outgammaseq(\ell),\epsilon)}}\geq\frac{1}{2}(\frac{\eulerv{d'\epsilon}}{r'(1+\frac{d''\epsilon}{2})})^\ell.$$  
%We claim that for any $s>0$, $\exists \ell,\epsilon$ such that
%$$\frac{1}{2}(\frac{\eulerv{d'\epsilon}}{r'(1+\frac{d''\epsilon}{2})})^\ell>\eulerv{s\epsilon}.$$
%Now the above inequality holds if 
%$$\frac{\eulerv{(d'\ell-s)\epsilon}}{(1+\frac{d'\epsilon}{2})^\ell}>2{r'}^\ell.$$ 
%
%Choose $\ell$ so that $d'\ell>s.$ Since the denominator of the left hand side term of the last
%inequality grows polynomially in $\epsilon$, while its numerator grows
%exponentially in $\epsilon$, it is easy to see that 
% $\exists
%  \epsilon_{0}>\epsilon_\ell$ such that
%  $$ \forall \epsilon\geq \epsilon_0, \:\frac{\eulerv{(d'\ell-s)\epsilon}}{(1+\frac{d'\epsilon}{2})^\ell}>2{r'}^\ell.$$
%This shows that $\cA$ is not differentially private.
%
%\red{What changes need to be made for non-input}
%\end{proof}

%\begin{definition}
%Let $\inalphaseq$ be an input sequence, $\outgammaseq$ an output sequence, such that there is a path $\rho$ from initial state $\qinit$
%with $\inseq(\rho)=\inalphaseq$ and $\outseq(\rho)=\outgammaseq.$ Given $\epsilon>0$, let $Y(\epsilon)$ be the random variable that models the value of the variable $\rvar$ 
%at the end of execution of $\rho.$  Let $\pdfassgn{\alpha}{\gamma}{z}$ be the probability density function of the random variable $Y(\epsilon).$ 
%\end{definition}
%
%\red{Sequences}
%
%\begin{lemma}
%\label{lem:if2main}
%A  {\dipa} $\cA$ is 
%not differentially private if  it has a {\criticalpair} of cycles $(C,C')$ such that $C$ is reachable from the initial state of $\cA.$   
%
%\end{lemma}
%
%\begin{proof}
%Let $\cA= \defaut.$
%Assume that $\cA$  has a {\criticalpair} of cycles $(C,C')$ such that $C$ is reachable from $\qinit.$
%Assume that $C$ is an {\lcycle} and $C'$ is a {\gcycle}. (The proof for
%the case when $C$ is a {\gcycle} and $C'$ is an {\lcycle} is similar but
%symmetric and is left out). Without loss of generality, we assume that
%neither $C$ nor $C'$ by themselves  are {{\criticalcycle}}s; otherwise, by
%Lemma  \ref{lem:if1main}, $\cA$ is not differentially private. This
%assumption means both $C,C'$ do not have assignment transitions. We
%further assume that $C,C'$ are distinct. If they are the same then it is
%straightforward to prove that $\cA$ is not differentially private,
%using  more or less the same proof. We also assume that all the states in $\cA$ are input states. The case when $\cA$ has both input and 
%non-input states can also be proved using more or less the same proof. 
%
%Let the lengths of $C,C'$ be $n_1,n_2$, respectively. 
%Now, for any $\ell>0$, consider the following abstract path $\absexec_{\ell}$ in $\cA$ starting
%from $\qinit$ in which the cycles $C,C'$ are repeated $\ell$ times
%each. The path
%$$\begin{array}{lcl}
%\absexec_{\ell}&=& q_0o_0 \cdots q_u o_u \cdots q_v o_v \cdots q_{v+n_1\ell-1} o_{v+n_1\ell-1}\cdots \\
%                        && \hspace*{1cm} \cdots q_{w}o_w\cdots o_{w+n_2\ell-1} q_{w+n_2\ell}
%\end{array}$$
%where the following conditions are satisfied. For each k, let $t_k$ be the $k$-th transition of $\absexec.$ and $c_k$ be the Boolean condition of the $k$-th transition.
%\begin{enumerate}
%\item $q_0=\qinit$
%\item $\absexecsf{v}{v+n_1}$ is the cycle C
%\item $t_{j+n_1}\:=t_{j}$ for all $j,\: v\leq j<v+n_1(\ell-1)$
%\item $\absexecsf{w}{w+n_2}$  is the cycle $C'$
%\item $t_{j+n_2}\:=t_{j}$ for all $j,\:w\leq j<w+n_2(\ell-1)$
%\item $t_u$ is an assignment transition and $\forall\:j,
%u<j<v+n_1\ell$ and $\forall\:j,
%j\geq w$, $t_j$ is a non-assignment transition
%\item for all
%$j,\:v+n_1\ell\leq j<w $, if $t_j$ is an assignment transition then
%$c_j$ is the condition $\getest.$
%
%\end{enumerate}
%%
%%$\absexec_{\ell}\:=(t_0,...,t_u,...,t_v,....,t_{v+n_1\ell-1},..,t_{w},...,t_{w+n_2\ell-1})$
%%where  $t_k\:=(q_k,a_k,o_k,f(a_k,\epsilon),c_k,A_k,q_{k+1})$, for
%%$0\leq k <w+n_2\ell$, $u\leq v$, $v+n_1\ell\leq w$ and the following conditions are satisfied: (i)
%%$q_0\:=\qinit$;(ii)  $(t_v,...,t_{v+n_1-1})$ is the cycle $C$ and
%%$q_v\:=q_{v+n_1}$; (iii) $t_{j+n_1}\:=t_{j}$ for all $j,\: v\leq
%%j<v+n_1(\ell-1)$; (iv) $(t_w,...,t_{w+n_2-1})$ is the cycle $C'$ and
%%$q_w\:=q_{w+n_2}$; (v) $t_{j+n_2}\:=t_{j}$ for all $j,\:w\leq
%%j<w+n_2(\ell-1)$; (vi) $t_u$ is an assignment transition and $\forall\:j,
%%u<j<v+n_1\ell$ and $\forall\:j,
%%j\geq w$, $t_j$ is a non-assignment transition; (vii) for all
%%$j,\:v+n_1\ell\leq j<w $, if $t_j$ is an assignment transition then
%%$c_j$ is the condition $\getest.$
% Observe that the last
%assignment transition before $t_{v+n_1\ell}$ is $t_u$, all assignment
%transitions from $t_{v+n_1\ell}$ up to $t_w$ have ${\getest}$ as
%their condition, the segment of the path from $t_v$ to
%$t_v+n_1\ell-1$ is the part where cycle $C$ is repeated $\ell$ times
%and the segment of the path from $t_w$ to
%$t_w+n_2\ell-1$ is the part where cycle $C'$ is repeated $\ell$ times.
%
%Let $d_k$ and $\mu_k$ be such that $\parf(q_k) = (d_k,\mu_k)$ for each $k.$
% \red{Without loss of generality}, we assume that
%$c_0\:=\true$ and  $t_0$ is an
%assignment transition.
%Now, we define two adjacent input sequences $\inalphaseq(\ell)=\inalpha_0\cdots\inalpha_{w+n_2\ell-1}$ and
%$\inbetaseq(\ell)\:=\inbeta_0\cdots\inbeta_{w+n_2\ell-1}$ as follows. For all
%$j,0\leq j< v$ and for all $j,\:v+n_1\ell \leq
%j<w$,$\inalpha_j\:=\inbeta_j\:=0$; for all $j,\:v\leq j<v+n_1\ell$ and  for all $j,\:w\leq
%j<w+n_2\ell$, if $c_j$ is the condition $\getest$ then
%$\inalpha_j\:=\frac{1}{2}-\mu_j,\: \inbeta_j\:=-\frac{1}{2}-\mu_j$, if $c_j$ is the
%condition  $\lttest$ then
%$\inalpha_j\:=-\frac{1}{2}-\mu_j,\: \inbeta_j\:=\frac{1}{2}-\mu_j$ and if $c_j$ is
%$\true$ then $\inalpha_j\:=\inbeta_j\:=0.$ It is not difficult to see that
%$\inalphaseq(\ell)$ and $\inbetaseq(\ell)$ are adjacent. Let
%$\outgammaseq(\ell)\:=o_0\cdots o_j\cdots$ be the sequence of outputs in the
%transitions of $\absexec_{\ell}.$
%
%Let $X_j,U_j$ be random variables with distributions given by
%$\Lap{d_{j}\epsilon,\inalpha_j+\mu_j}$ and
%$\Lap{d_{j}\epsilon,\inbeta_j+\mu_j}$, respectively. 
%Recall that $\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{z}$ is the p.d.f of
%the random variable that models the value of $\rvar$ after $\ell$  steps of  $\absexec$ on input $\inalphaseq.$ 
%Since $\inalphaseq(\ell)|v\:=\inbetaseq(\ell)|v$ we see
%that $\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{z}\:=
%\pdfassgn{\inbetaseq(\ell)|v}{\outgammaseq(\ell)|v}{z}.$ Observe that $t_u$
%is the last assignment transition in $\absexec_{\ell}.$ For each $j>u$, for any
%given $y\in \Reals$, let
%$g_j(y),h_j(y)$ be the probabilities defined as follows: if $c_j$ is
%the condition ${\getest}$ then $g_j(y)\:=\prbfn{X_j\geq y}$ and 
%$h_j(y)\:=\prbfn{U_j\geq y}$; if $c_j$ is
%the condition $\lttest$ then $g_j(y)\:=\prbfn{X_j< y}$ and 
%$h_j(y)\:=\prbfn{U_j< y}$; if $c_j$ is $\true$ then
%$g_j(y)\:=h_j(y)\:=1.$ It should be easy to see that,  for  all $j,\:u<j<v$ and for all $j,\:v+n_1\ell \leq
%j<w$,
%$\inalpha_j\:=\inbeta_j$ and hence
%$g_j(y)\:=h_j(y).$
%Now, we have the following claim.
%
%%Let $z$ be a
%%variable taking values from $\Reals$ and $\rho_z$ be the evaluation
%%where $\rho(x)\:=z.$ From our definitions, we see that
%%$\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{z}$ is the probability
%%that $\cA$ on the input sequence $\inalphaseq(\ell)|v$ outputs $\outgammaseq(\ell)|v$
%%under the condition that the variable $x$ has value $z$ at the end of the
%%input $\inalphaseq(\ell)|v.$ Since $\inalphaseq(\ell)|v\:=\inbetaseq(\ell)|v$ we see
%%that $\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{z}\:=
%%\pdfassgn{\inbetaseq(\ell)|v}{\outgammaseq(\ell)|v}{z}.$ Observe that $t_u$
%%is the last assignment transition in $\absexec_{\ell}.$ For each $j>u$, for any
%%given $y\in \Reals$, let
%%$g_j(y),h_j(y)$ be the probabilities defined as follows: if $c_j$ is
%%the condition ${\getest}$ then $g_j(y)\:=\prbfn\{X_j\geq y\}$ and 
%%$h_j(y)\:=\prbfn\{U_j\geq y\}$; if $c_j$ is
%%the condition $\lttest$ then $g_j(y)\:=\prbfn\{X_j< y\}$ and 
%%$h_j(y)\:=\prbfn\{U_j< y\}$; if $c_j$ is $\true$ then
%%$g_j(y)\:=h_j(y)\:=1.$ It should be easy to see that,  for  all $j,\:u<j<v$ and for all $j,\:v+n_1\ell \leq
%%j<w$,
%%$\inalpha_j\:=\inbeta_j$ and hence
%%$g_j(y)\:=h_j(y).$
%%Now, we have the following claim.
%
%{\bf Claim:} For all $j, v\leq j <v+n_1\ell$, and for all
%$j,\:w\leq j<w+n_2\ell$, it is the case that $g_j(y)\geq h_j(y)$ for
%all $y\in \Reals$, and the following
%additional inequalities hold.
% 
%\begin{enumerate}
%
%\item If $y\leq 0$ and  $c_j$ is the condition $\lttest$  then $g_j(y)
%    \geq \eulerv{\frac{1}{2}d_{j}\epsilon}h_j(y).$ 
%
%\item  If $y>0$ and $c_j$ is the condition
%  ${\getest}$ then  $g_j(y)
%    \geq \eulerv{\frac{1}{2}d_{j}\epsilon}h_j(y).$
%
%\end{enumerate}
%
%\begin{proof}
% Observe that when $c_j\:=\true$
%then trivially $g_j(y)\:=h_j(y).$ Now, consider the case when
%$y<-\frac{1}{2}.$ If $c_j$ is the condition $\getest$ then
%$g_j(y)\:= 1-\frac{1}{2}\eulerv{-d_{j}\epsilon(\frac{1}{2}-y)}$ and
%$h_j(y)\:=1-\frac{1}{2}\eulerv{-d_{j}\epsilon(-\frac{1}{2}-y)}$(this
%is so since $\inalpha_j+\mu_j=\frac{1}{2}$ and $\inbeta_j+\mu_j=-\frac{1}{2}$) ; in
%this case $\frac{1}{2}-y>-\frac{1}{2}-y$ and hence $g_j(y)\geq
%h_j(y).$ If $c_j$ is the condition $\lttest$ then $g_j(y)\:=
%\frac{1}{2}\eulerv{-d_{j}\epsilon(-\frac{1}{2}-y)}$ and
%$h_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(\frac{1}{2}-y)}$; from
%this we see that $g_j(y)\geq  \eulerv{d_{j}\epsilon}h_j(y).$
%
%Now consider the case when $y\in [-\frac{1}{2},0].$ If $c_j$ is the
%condition $\getest$ then
%$g_j(y)\:= 1-\frac{1}{2}\eulerv{-d_{j}\epsilon(\frac{1}{2}-y)}$ and
%$h_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(y+\frac{1}{2})}$;
%since $g_j(y)\geq \frac{1}{2}$ and $h_j(y)\leq \frac{1}{2}$, we see that $g_j(y)
%    \geq h_j(y).$   If $c_j$ is the
%condition $\svar < x$ then 
%$g_j(y)\:= 1-\frac{1}{2}\eulerv{-d_{j}\epsilon(y+\frac{1}{2})}$
%and $h_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(\frac{1}{2}-y)}$;
%since $g_j(y)\geq \frac{1}{2}$, we see that $g_j(y)\geq
%\eulerv{\frac{1}{2}d_{j}\epsilon}h_j(y).$
%
%Now consider the case when $y>0.$ If $y\leq \frac{1}{2}$ and $c_j$ is
%${\getest}$ then $g_j(y)\:=
%1-\frac{1}{2}\eulerv{-d_{j}\epsilon(\frac{1}{2}-y)}$ and 
%$h_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(y+\frac{1}{2})}$;
%observe that $g_j(y)\geq \frac{1}{2}$ and $h_j(y)\leq
%\frac{1}{2}\eulerv{-\frac{1}{2}d_{j}\epsilon}$; from this we get the desired
%  inequality. 
%
%If $y\leq \frac{1}{2}$ and $c_j$ is
%$\lttest$ then $g_j(y)\:=
%1-\frac{1}{2}\eulerv{-d_{j}\epsilon(y+\frac{1}{2})}$ and $h_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(\frac{1}{2}-y)}$; since $g_j(y)\geq \frac{1}{2}$ and $h_j(y)\leq \frac{1}{2}$, we see $g_j(y)\geq h_j(y).$ If $y>\frac{1}{2}$ and $c_j$ is 
%${\getest}$ then
%$g_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(y-\frac{1}{2})}$ and
%$h_j(y)\:=\frac{1}{2}\eulerv{-d_{j}\epsilon(y+\frac{1}{2})}$; from
%this we see that the
%desired inequality follows easily. If $y>\frac{1}{2}$ and $c_j$ is 
%$\lttest$ then
%$g_j(y)\:=1-\frac{1}{2}\eulerv{-d_{j}\epsilon(y+\frac{1}{2})}$ and
%$h_j(y)\:=1-\frac{1}{2}\eulerv{-d_{j}\epsilon(y-\frac{1}{2})}$; it
%is easy to see that $g_j(y)\geq h_j(y).$
%\end{proof}
%
%Let $S_1(\ell)$ be the set of all $j$ such that  $v\leq j<v+n_1\ell$
%and $c_j$ is the condition $\svar < x.$ 
%Let $S_2(\ell)$ be the set of all $j$ such that  
%$w\leq j<w+n_2\ell$, and $c_j$ is the condition ${\getest}.$ 
%Since $C$ is an {\lcycle} and $C'$ is a {\gcycle}, we see that the
%cardinalities of both $S_1(\ell)$ and $S_2(\ell)$ are $\geq \ell.$
% Let $d_{\min}\:= \min\set{d_{j}\st j\in
%  S_1(\ell)\cup S_2(\ell)}.$ Clearly $d_{\min}>0.$ 
%
%%WIth out loss of generality, we assume that
%%$inseq(\exec_{\ell})\:=\inalphaseq(\ell).$ Let $\exec'_{\ell}$ be a path equivalent
%%to $\exec_{\ell}$ such that $inseq(\exec'_{\ell})\:=\inbetaseq(\ell).$ Recall that
%%$\exec_{\ell}||w$ is the suffix of $\exec_{\ell}$ starting with $t_w$ and it
%%is of length $n_2\ell.$
%
%Let $\exec_\ell=\absexec[\inalphaseq]$ be the path that results from the execution of 
%$\absexec$ on input $\inalphaseq.$  Let $\exec'_\ell=\absexec[\inbetaseq]$ be the path that results from the execution of 
%$\absexec$ on input $\inbetaseq.$ Recall that
%$\exec_{\ell}||w$ is the suffix of $\exec_{\ell}$ starting with $q_w$ and it
%is of length $n_2\ell.$
%
%
%Since $C'$ is a {\gcycle}, from the above claim, we see that 
%$\forall y\in \Reals$, $\pathprob{\exec_{\ell}||w,y}\geq
%\pathprob{\exec'_{\ell}||w,y}$,  and $\forall y>0$, $\pathprob{\exec_{\ell}||w,y}\geq
%\eulerv{\frac{1}{2}d_{\min}\ell\epsilon}\pathprob{\exec'_{\ell}||w,y}.$ Using the
%above property and the previous  claim, together with the
%assumption that 
%$\forall j,\:v+n_1\ell\leq j<w$, if $t_j$ is an assignment transition
%then it's condition is $\getest$, the following can be proved
%by downward induction on $k$,  $\forall k,\:v+n_1\ell \leq k <w$: 
%$\forall y\in \Reals$, $\pathprob{\exec_{\ell}||k,y}\geq
%\pathprob{\exec'_{\ell}||k,y}$,  and $\forall y>0$, $\pathprob{\exec_{\ell}||k,y}\geq
%\eulerv{\frac{1}{2}d_{\min}\ell\epsilon}\pathprob{\exec'_{\ell}||k,y}.$
%
%Now, it should be easy to see that $\forall y\in\Reals,$
%$$
%\begin{array}{lcl}
%\pathprob{\exec_{\ell}||v,y} &=&  (\prod_{v\leq  j<v+n_1\ell}g_j(y)) 
%\pathprob{\exec_{\ell}||v+n_{1}\ell,y} \\
%\pathprob{\exec'_{\ell}||v,y} &=& (\prod_{v\leq  j<v+n_1\ell}h_j(y)) 
%\pathprob{\exec'_{\ell}||v+n_{1}\ell,y}.
%\end{array}$$
% Observe that $\forall
%j,\: v\leq  j<v+n_1\ell,$
%$$\forall y\leq 0: g_j(y)\geq
%\eulerv{\frac{1}{2}d_{\min}\epsilon} h_j(y),\: \pathprob{\exec_{\ell}||j,y}\geq
%\pathprob{\exec'_{\ell}||j,y}$$ 
%and 
% $$\forall y>0,\: g_j(y)\geq h_j(y),\: \pathprob{\exec_{\ell}||j,y}\geq
%\eulerv{\frac{1}{2}d_{\min}\ell \epsilon} \pathprob{\exec'_{\ell}||j,y}.$$
%From this we get the
%following: $$\forall y\in \Reals,\: \pathprob{\exec_{\ell}||v,y}\geq
%\eulerv{\frac{1}{2}d_{\min}\ell \epsilon} \pathprob{\exec'_{\ell}||v,y}.$$
%
% 
% Now, we observe that 
% $$
% \begin{array}{l}
% \red{\Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)}= \int^{\infty}_{-\infty}
%\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{y} \pathprob{\exec_{\ell}||v,y}dy.\\
%\red{ \Pr(\inbetaseq(\ell),\outgammaseq(\ell),\epsilon)}= \int^{\infty}_{-\infty}
%\pdfassgn{\inbetaseq(\ell)|v}{\outgammaseq(\ell)|v}{y} \pathprob{\exec'_{\ell}||v,y}dy.\\
% \end{array}
% $$
%
%From the facts that $\pathprob{\exec_{\ell}||v,y}
%\geq \eulerv{\frac{1}{2}d_{\min}\ell\epsilon}\pathprob{\exec'_{\ell}||v,y}$ and that $\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{y}\:=
%\pdfassgn{\inbetaseq(\ell)|v}{\outgammaseq(\ell)|v}{y}$, we see
%that
%$\frac{\red{\Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)}}{\red{\Pr(\inbetaseq(\ell),\outgammaseq(\ell),\epsilon)}}\geq
%\eulerv{\frac{1}{2}d_{\min}\ell\epsilon}.$ Since  $\ell$ can be made arbitrarily large, we see that $\cA$ is not
%$a\epsilon$-differentially private, for any $a>0$. Hence $\cA$ is not
%differentially private. 
%\end{proof}

% 
% Note that $\inalpha_u\:=\inbeta_u\:=0$ and both $X_u,U_u$ are random
%variables with distribution $\Lap{d_{u}\epsilon,0}$ which is
%  given by the probability density function
%  $\psi(y)\:=\frac{d_{u}\epsilon}{2}\eulerv{-d_{u}\epsilon
%    y}.$ 
%    Recall that $t_u$
%  is the last assignment transition before $t_{v+n_{1}\ell}.$ Now, we see that 
%$$\Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)\:=\int^{\infty}_{-\infty}
%\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{y} \psi(y)\pathprob{\exec_{\ell}||v,y}dy,$$
%$$\Pr(\inbetaseq(\ell),\outgammaseq(\ell),\epsilon)\:=\int^{\infty}_{-\infty}
%\pdfassgn{\inbetaseq(\ell)|v}{\outgammaseq(\ell)|v}{y} \psi(y)\pathprob{\exec'_{\ell}||v,y} dy.$$

%Since $\pdfassgn{\inalphaseq(\ell)|v}{\outgammaseq(\ell)|v}{y}\:=
%\pdfassgn{\inbetaseq(\ell)|v}{\outgammaseq(\ell)|v}{y}$ and $\pathprob{\exec_{\ell}||v,y}
%\geq \eulerv{\frac{1}{2}d_{\min}\ell\epsilon}\pathprob{\exec'_{\ell}||v,y}$, we see
%that
%$\frac{\Pr(\inalphaseq(\ell),\outgammaseq(\ell),\epsilon)}{\Pr(\inbetaseq(\ell),\outgammaseq(\ell),\epsilon)}\geq
%\eulerv{\frac{1}{2}d_{\min}\ell\epsilon}.$ Since  $\ell$ can be made arbitrarily large, we see that $\cA$ is not
%$a\epsilon$-differentially private, for any $a>0$. Hence $\cA$ is not
%differentially private.

%\subsection{Sufficient Condition for Differential Privacy}
%
%Assume that $\cA = (Q,\Sigma,O,X,\delta,F,\qinit)$ is a well-formed
%{\dipa},that is, it   
% has no {\criticalcycle}  reachable from $\qinit$ and it has no critical 
%pair of cycles $(C,C')$ such that $C$ is reachable from $\qinit.$
%Without loss of generality, we assume that all states of $\cA$ are
%reachable fromm the initial state $\qinit.$
%A transition  is called a {\em critical transition}, if it does not lie
%on a cycle in $\cA$. A transition that lies on an {\lcycle} or a {\gcycle},
%is respectively called an {\lcycle}  or a {\gcycle} transition. Observe
%that an assignment transition cannot be an {\lcycle} or a {\gcycle}
%transition since that will make that cycle a {\criticalcycle} and $\cA$
%will not be well-formed. An assignment transition can lie on a cycle
%which is neither an {\lcycle} nor a {\gcycle}, i.e., all the transitions
%on such cycle have the condition $\true.$ Observe that $\cA$ can not
%have a cycle that is both an {\lcycle} and a {\gcycle}, since in that
%case $\cA$ will not be well-formed.
% 
%Consider a path $p$ given by the sequence of transitions
% $(q_i,a_{i},o_{i},f(a_{i},\epsilon),c_i,A_i,q_{i+1})$, for
%$i=0,...,n-1$ for some $n>0.$ We define $weight(p)$ to be the sum
%of $d_{j}$ for all $j$ such that $0\leq j\leq n$, and $t_j$ is a
%critical transition.
%\begin{lemma}
%\label{lem:integralineq}
%Let $f$ and $g$  be positive functions from $\Reals$ to $\Reals$, i.e.,
%$f(y),g(y)\geq 0$ for all $y\in \Reals.$ For $i=1,...,k$, let $\theta_i\in
%[-1,1]$.
%Let $x_0,x_1\in Reals\cup \set{\infty,-\infty}$, be such that $x_0<x_1$.
%Then, the following inequalities
%are satisfied for all $k\geq 0$. For the case when $k=0$, the products
%$\prod^k_{i=1}$, in these inequalities are taken be $1.$
%
%\begin{enumerate}
%\item $\displaystyle{\int^{x_{1}}_{x_{0}}\:f(x) 
%  \prod^k_{i=1}\int^\infty_x\:g_i(y-\theta_i)dy dx\;\geq \int^{x_{1}+1}_{x_{0}+1}\:f(x-1) 
%  \prod^k_{i=1}\int^\infty_x\:g_i(y)dy\: dx}$
%\item $\displaystyle{\int^{x_{1}}_{x_{0}}\:f(x) 
%  \prod^k_{i=1}\int^x_{-\infty}\:g_i(y-\theta_i)dy dx\;\geq \int^{x_{1}-1}_{x_{0}-1}\:f(x+1) 
%  \prod^k_{i=1}\int^x_{-\infty}\:g_i(y)dy\: dx}$
%\end{enumerate}
%\end{lemma}
%\begin{proof}
%We prove the inequality (1) as follows. For each $i=1,...,k$, by substituting
%$z\:=y-\theta_i$, we get $\int_x^\infty  g_i(y-\theta_i)dy
%\:=\int^\infty_{x-\theta_i}g_i(z)dz.$ Since $\theta_i\in [-1,1]$ and
%$g_i$ is a positive function, we get
%$\int^\infty_{x-\theta_i}g_i(z)dz\:\geq \int^\infty_{x+1}g_i(z)dz.$ By
%rewriting the left hand side of the inequality (1) as specified above
%and by substituting, $u = x+1$, we get the right hand side of the
%inequality (1) where the outer integral is over the variable $u.$ By
%replacing $u$ by $x$ and $z$ by $y$, we get the right hand side of the
%inequality. 
%
%We prove the inequality (2) as follows. As before, for each
%$i=1,...,k$, we rewrite the integral $\int^x_{-\infty}
%g_i(y-\theta_i)dy$ as $\int^{x-\theta_i}_{-\infty}
%g_i(z)dz$ and then observe that this is $\geq \int^{x-1}_{-\infty}
%g_i(z)dz.$ Substituting $u\:=x-1$, and then replacing $u$ by $x$ later,
%we get the inequality (2).
%
% 
%\end{proof}
%
%\begin{lemma}
%\label{lem:main}
%Let $\cA$ be a well-formed SVT-automaton as specified above. Let  $p= (t_0,...,t_{n-1})$ be a path of length $n>0$, where
%$t_i=(q_i,a_i,o_if(a_i,\epsilon),c_i,A_i,q_{i+1})$ for $0\leq
%i<n$ and $t_0$ is an assignment transition. 
%%Further assume that the
%%suffix of $p$ starting with $t_1$, i.e., the suffix $p||1$, has no
%%assignment transitions whose condition is $\true.$
%Let $p'$ be a path that is equivalent  to $p$ such that
%$inseq(p')\:=(b_0,...,b_{n-1})$ is a neighbour of $inseq(p).$ Then the following properties
%hold for all $x_0\in \Reals.$ 
%\begin{enumerate}
%\item  If the condition $c_0$ is $\getest$,  and  the first
%  cycle transition in $p$ is a {\gcycle} transition and no assignment
%  transition 
%with condition   $\lttest$ appears before it, then 
%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon} G_{p}(x_0+1).$$
%%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon}\int^{\infty}_{x_{0}+1}
%%d_{q_{0}}\frac{\epsilon}{2}\eulerv{-d_{q_{0}}\epsilon|x-a_{0}|}G_{p||1}(x) 
%%dx.$$
%\item  If the condition $c_0$ is $\getest$ and one of the
%  following holds:  (a) $p$ has no cycle transitions,  (b)  the first
%  cycle transition in $p$ is a  {\gcycle} transition and an assignment transition with condition 
%  $\lttest$ appears before it,  (c) the first cycle transition
%  in $p$ is an {\lcycle} transition,
%  then
%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon} G_p(x_{0}-1). 
%$$
%%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon}\int^{\infty}_{x_{0}-1}
%%d_{q_{0}}\frac{\epsilon}{2}\eulerv{-d_{q_{0}}\epsilon|x-a_{0}|}G_{p||1}(x) 
%%dx.$$ 
%
%\item  If the condition $c_0$ is $\svar < x$  and the first cycle
%  transition in $p$ is a 
%{\lcycle}   transition  and  no assignment transition with condition 
%  $\getest$ appears before it, then 
%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon}G_p(x_0-1).$$
%%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon}\int^{x_{0}-1}_{-\infty}
%%d_{q_{0}}\frac{\epsilon}{2}\eulerv{-d_{q_{0}}\epsilon\mathbin{|}x-a_{0}\mathbin{|}}G_{p%||1}(x) 
%%dx.$$
%\item  If the condition $c_0$ is $\svar < x$ and one of the
%  following holds: (a) $p$ has no cycle transitions, (b) the first
%  cycle transition in $p$  is  a 
%{\lcycle}   transition  and an assignment transition with condition 
%  $\getest$ appears before it, (c) the first cycle
%  transition in $p$ is a {\gcycle} transition, then 
%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon}G_p(x_0+1).$$
%%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon}\int^{x_{0}+1}_{-\infty}
%%d_{q_{0}}\frac{\epsilon}{2}\eulerv{-d_{q_{0}}\epsilon\mathbin{|}x-a_{0}\mathbin{|}}G_{p%||1}(x) 
%%dx.$$
%
%\item If the condition $c_0$ is $\true$, then $G_{p'}(x_0)\geq
%  \eulerv{-2weight(p)\epsilon} G_p(x_0).$
%\end{enumerate}
%\end{lemma}
%\begin{proof}
%Let $p||1$ denote the
%suffix of $p$ starting from $t_1.$
%For each $k$, such that $0\leq k<n$, let $g_k,g'_k$ be functions of a
%single variable given by
%$g_k(y)\:=\frac{d_{q_{k}}\epsilon}{2}\eulerv{-d_{q_{k}}\epsilon\mathbin{|}y-a_k\mathbin{|}}$,
%$g'_k(y)\:=\frac{d_{q_{k}}\epsilon}{2}\eulerv{-d_{q_{k}}\epsilon\mathbin{|}y-b_k\mathbin{|}}$
%and $\theta_k\:=b_k-a_k.$ Observe that, for each $k\geq 0$, $g'_k(y)\:=g_k(y-\theta_k).$ Since $\card{\theta_k}\leq 1$, we see that
%$g'_k(y)\geq \eulerv{-d_{q_{k}}\epsilon}g_k(y)$, for all $y\in \Reals.$
%
%We prove the lemma by induction on the number of assignment
%transitions in $p.$ In the base case, $p$ has one assignment
%transition which is $t_0.$ Let
%$S_1$ and $S_2$  be the sets of $k>0$ such that $c_k$ is $\svar
%\geq x$ and $c_k$ is $\svar < x$, respectively. Now, assume the condition of (1) is
%satisfied. Observe that $S_1$ includes
%all {\gcycle} transition whose condition  is $\getest.$ Observe that, since
%$\cA$ is well-formed, for all
%$k\in S_2$, $t_k$ does not lie on a cycle and hence is a critical
%transition. Similarly $t_0$ is also a critical transition. 
%Now, we see 
%that $$G_{p'}(x_0)\:=\:\int^\infty_{x_{0}}f(x)\prod_{k\in 
%    S_{1}}\int^\infty_xg'_k(y) dy\:  dx$$ where 
%$\displaystyle{f(x)\:=\:g'_0(x)\prod_{k\in 
%      S_{2}}\int^x_{-\infty} g'_k(y) dy}.$
%Now, using inequality
%  (1) of Lemma \ref{lem:integralineq}, we see that
%  $\displaystyle{G_{p'}(x_0)\geq\int^\infty_{x_{0}+1}f(x-1)\prod_{k\in
%      S_{1}}\int^\infty_xg_k(y)dy\:dx}.$ Now, observe that
%    $f(x-1)\:=g_0(x-(1+\theta_0))\prod_{k\in
%      S_{2}}\int^{x-1}_{-\infty}g_k(y-\theta_k) dy.$ Now, by
%    introducing a new variable $z$ such that $z\:=y+1$, we see that
%    $\int^{x-1}_{-\infty}g_k(y-\theta_k) dy\:=
%    \int^{x}_{-\infty}g_k(z-(1+\theta_k)) dz..$
%From this, it is easy to see that  we see that $f(x-1)\geq
%\eulerv{-2(d_{q_{0}}+\sum_{k\in
%    S_{2}}d_{q_{k}})\epsilon}g_0(x)\prod_{k\in
%  S_{2}}\int^{x}_{-\infty}g_k(y) dy$. 
%Observe that $weight(p)\:\geq d_{q_{0}}+\sum_{k\in S_{2}}d_{q_{k}}.$
%Putting all the above observations together, we get 
%$$G_{p'}(x_0)\geq \eulerv{-2weight(p)\epsilon} \int^\infty_{x_{0}+1
%}g_0(x)\prod_{k\in S_2}\int^x_{-\infty}g_k(y) dy\:\prod_{k\in S_{1}}
%\int^\infty_xg_k(y) dy$$
%By observing that $G_{p||1}(x)\:=\prod_{k\in S_2}\int^x_{-\infty}g_k(y) dy\:\prod_{k\in S_{1}}
%\int^\infty_xg_k(y) dy$,
%we see that property (1) of the lemma follows for the base case.  
%
%Now, we prove the base case for property (2). Assume the condition of
%(2a) is satisfied,i.e., there are no cycle transitions in $p.$ Now, we see that 
%$$G_{p'}(x_0)\:=\:\int^\infty_{x_{0}}g'_0(x)\prod_{k\in 
%    S_{1}}\int^\infty_xg'_k(y) dy \prod_{k\in 
%    S_{2}}\int^x_{-\infty}g'_k(z) dz\:dx.$$
%By introducing new variables $u,v,w$ such $u\:=x-1,\:v=y-1,\:w=z-1$,
%we get  
%$$G_{p'}(x_0)\:=\:\int^\infty_{x_{0}-1}g'_0(u+1)\prod_{k\in 
%    S_{1}}\int^\infty_ug'_k(v+1) dv \prod_{k\in 
%    S_{2}}\int^u_{-\infty}g'_k(w+1) dw\:du.$$
%Observing that, for each $k\geq 0$, $g'_k(u+1)\geq
%\eulerv{-2d_{q_{k}}\epsilon}g_k(u)$ and $t_k$ is a critical
%transition, we get the inequality of property (2). 
%
%Now observe that condition of (2b) can not be satisfied as $t_0$ is the only assignment transition in
%$p$. Now, assume the condition of (2c) is satisfied.  
%Now, observe that, for all $k\in S_1$, $t_k$ is a critical
%transition. As before, we see that 
%that $$G_{p'}(x_0)\:=\:\int^\infty_{x_{0}}f(x)\prod_{k\in S_{2}}\int^x_{-\infty} g'_k(y) dy\: h(x) dx$$ where 
%$\displaystyle{f(x)\:=\:g'_0(x)\prod_{k\in 
%      S_{1}}\int^\infty_x g'_k(y) dy}.$  Now, using inequality
%  (2) of Lemma \ref{lem:integralineq}, we see that
%  $\displaystyle{G_{p'}(x_0)\geq\int^\infty_{x_{0}-1}f(x+1)\prod_{k\in
%      S_{2}}\int^x_{-\infty} g_k(y)dy\:dx}.$ Now, observe that
%    $f(x+1)\:=g_0(x-(\theta_0-1))\prod_{k\in S_{1}}\int_x^\infty g_k(y-(\theta_k-1))dy$
%      and
%$f(x+1)\geq \eulerv{-2(d_{q_{0}}+\sum_{k\in
%    S_{2}}d_{q_{k}})\epsilon}g_0(x)\prod_{k\in S_{1}}\int_x^\infty g_k(y)dy$. The
%required result follows from this.
%The proof for the base case of Properties (3) and (4) is symmetric to
%those of properties (1) and (2) and is left out. To prove property (5)
%for the base case, we see that the proof is similar to those of
%properties (1) and (3) depending on whether {\gcycle} or {\lcycle}
%transitions appear. The only difference being, the lower limit of the
%outer integral will be $-\infty$ in the former case, while the upper
%limit of the outer integral being $\infty$ in the later case. In
%either case, it is straightforward to see that property (5) holds.
%
%Now, we prove the inductive step as follows. Assume that all the
%properties hold when $p$ has $\ell>0$ assignments. Now, consider the
%case when $p$ has $\ell+1$ assignments. Let $t_i$, for $i>0$, be the
%second assignment transition in $p.$ 
%Let $S_1$ (resp., $S_2$) be the set of $k$, $0<k<i$, such that $c_k$ is $\svar
%\geq x$ (resp., $\lttest$).
%Let $S\:=\set{k\::0< k<i,\:c_k\neq \true}.$ 
%Now, consider the case when $c_0$
%is $\getest.$
%Now, we consider two sub-cases. We first consider the sub-case, which
%is, when there is no cycle transitions before $t_i.$
%We have $G_{p'}(x_0)\:=\int^\infty_{x_{0}}f'(x) 
%G_{p'||i}(x) dx$ where 
%$f'(x) \:=g'_0(x)\prod_{k\in S_{1}}\int_x^{\infty}g'_k(y)dy\prod_{k\in S_{2}}\int^x_{-\infty}g'_k(y)dy.$ 
% Applying the
%inductive hypothesis for the suffix $p||i$, we get an inequality
%involving $G_{p'||i}(x)$ and $G_{p||i+1}(x)$, based on which of  the five properties
%of the lemma are satisfied. Suppose the condition of property (1) is
%satisfied for $p||i$, by using the inductive hypothesis,  we get
%$\displaystyle{G_{p'}(x_0)\geq \int^{\infty}_{x_{0}} f'(x) h(x) dx}$, 
%where $$h(x)\:= \eulerv{-2weight(p||i)\epsilon}\int^\infty_{x+1}
%d_{q_{i}}\frac{\epsilon}{2}\eulerv{-d_{q_{i}}\epsilon|y-a_{i}|}G_{p||i+1}(y) 
%dy .$$ 
%Now, by taking $f(x)\:=f'(x)h(x)$, using inequality (1) of Lemma
%\ref{lem:integralineq} and by taking
%$k=0$ in that inequality, we get property (1) for the path $p$
% using the same simplification, reasoning as in the base case and by
% observing that $\displaystyle{G_{p||1}(x)\:=  \prod_{k\in
%     S_1}\int_x^{\infty}g_k(y)dy\prod_{k\in S_{2}}\int^x_{-\infty}g_k(y)dy
%   \int_x^\infty g_i(y) G_{p||i+1}(y) dy}.$ 
%We can similarly prove the inductive step when the suffix $p||i$
%satisfies the other properties (i.e., 2 through 5) of the lemma.
% Now consider the sub-case when a cycle transition appears before
%$t_i.$ Assume  that
%the cycle transitions are {\gcycle} transitions. If $c_i$ is also
%${\getest}$, then the suffix $p||i$ can satisfy any of the
%conditions of the first two properties of the lemma; In this
%situation, let 
%$f(x)\:=f'(x)h(x)$ where $f'(x)\:=g'_0(x)\prod_{k\in S_{2}}\int^x_{-\infty}g'_k(y)dy$
%and the function $h(x)$
%is defined as follows: if $p||i$ satisfies the condition of property (1)
%then $h(x)$ is the right handside of the inequality obtained by
%applying the inductive hypothesis to $p||i$ (i.e.,  $h(x)\:=\eulerv{-2weight(p||i)\epsilon}\int^{\infty}_{x+1}
%d_{q_{i}}\frac{\epsilon}{2}\eulerv{-d_{q_{i}}\epsilon|z-a_{i}|}G_{p||i+1}(z)
%dz$); If $p||i$ satisfies the condition of property (2) of the lemma
%then, by applying the inductive hypothesis to $p||i$, we get 
%$G_{p'||i}(x)\geq \eulerv{-2weight(p||i)\epsilon}\int^{\infty}_{x-1}
%d_{q_{i}}\frac{\epsilon}{2}\eulerv{-d_{q_{i}}\epsilon|z-a_{i}|}G_{p||i+1}(z) 
%dz$; for this case also, we take $h(x)\:=\eulerv{-2weight(p||i)\epsilon}\int^{\infty}_{x+1}
%d_{q_{i}}\frac{\epsilon}{2}\eulerv{-d_{q_{i}}\epsilon|z-a_{i}|}G_{p||i+1}(z) 
%dz$; observe that the earlier inequality implies that 
% $G_{p'||i}(x)\geq h(x).$ 
%Now, we have $G_{p'}(x_0)\:\geq \int^\infty_{x_{0}}f'(x)h(x)\prod_{k\in
%  S_{1}}\int^\infty_{x}g'_k(z) dz dx.$
%Applying the  inequality (1) of
% Lemma \ref{lem:integralineq}, we get the desired result for the
% inductive step.
%On the other hand, if $c_i$ is $\lttest$ then the suffix
%$p||i$ can not satisfy the condition of property (3) of the lemma due
%to wellformedness of $\cA$; however it can satisfy the condition of
%property (4). In this sub-case also, we can
%get the result for the induction case as above by using the inductive
%hypothesis for $p||i$ and using similar reasoning as in the base
%case and applying the first inequality of  Lemma
%\ref{lem:integralineq}. 
%
%Now consider the situation where  the cycle transitions appearing
%before $t_i$ are  {\lcycle} transitions. Now, we apply
%inequality (2) of Lemma \ref{lem:integralineq} to prove that property
%(2) of the lemma is satisfied by $p.$ To do this, we define $f(x)\:=f'(x)h(x)$
%where $f'(x)\:=g'_0(x)\prod_{k\in S_{1}}\int_x^{\infty}g'_k(y)dy$ and
%$h(x)$ is as given below. We apply the induction
%hypothesis to $p||i$ and   define $h(x)$, depending on which condition of
%five properties of the lemma is satisfied by
%$p||i$. Since $\cA$ is wellformed, $p||i$ cannot satisfy the condition
%of property (1)
%of the lemma.
%If $p||i$ satisfies the condition
%of property (2) then $h(x)\:= \eulerv{-2weight(p||i)\epsilon}\int^{\infty}_{x-1}
%d_{q_{i}}\frac{\epsilon}{2}\eulerv{-d_{q_{i}}\epsilon|z-a_{i}|}G_{p||i+1}(z)
%dz$; if  $p||i$ satisfies the condition
%of property (3) or (4) then $h(x)\:= \eulerv{-2weight(p||i)\epsilon}\int^{x-1}_{-\infty}
%d_{q_{i}}\frac{\epsilon}{2}\eulerv{-d_{q_{i}}\epsilon|z-a_{i}|}G_{p||i+1}(z)
%dz$; if $p||i$ satisfies the condition
%of property (5)  then $h(x)\:=
%\eulerv{-2weight(p||i)\epsilon}G_{p||i}(x-1).$ Observe that in the
%last case, i.e. when $p||i$ satisfies the condition of property (5),
%$h(x)$ is independent of $x$ since condition $c_i$ is $\true.$ By
%using the induction hypothesis, in all the above cases, it is easy to
%see that $G_{p'||i}(x)\geq h(x).$ Now, using the induction hypothesis, we get
%$G_{p'}(x_0)\:\geq \int^\infty_{x_{0}}f'(x)h(x)\prod_{k\in
%  S_{2}}\int^x_{-\infty}g'_k(z) dz dx.$ Now, using the inequality (2) of
%Lemma  \ref{lem:integralineq}, and using simplifications and reasoning
%as in the base cases, we see that property (2) of the lemma
%is satisfied by $p.$
%
%
%The proof for the inductive step for the case when $c_0$ is
%$\lttest$ is symmetric. For the case, when $c_0$ is $\true$, the
%proof will be on the same lines excepting that the limits of the outer
%integral are $-\infty$ and $\infty.$
%
%
%\end{proof}
%
%
%
%
%
%\begin{lemma}
%\label{lem:onlyifmain}
%If the  {\dipa} $\cA = (Q,\Sigma,O,X,\delta,F,\qinit)$  
%is well-formed then it is differentially private.  
%
%\end{lemma}
%\begin{proof}
%Assume that $\cA$, as given in the lemma, is well-formed. 
% Now, let $weight(\cA)$ be the maximum of $weight(p)$,
%where the maximum is taken over all paths $p$ in $\cA$ starting from
%$\qinit.$ We show that $\cA$ is $(2weight(\cA)\epsilon)$-differentially private. Consider any path
%starting from $\qinit.$ The first transition on all these paths has
%condition $\true.$ Applying the property (5) of Lemma \ref{lem:main},
%we get the desired result.
%
%
%\end{proof}
%
%

